Just Rotate it: Deploying Backdoor Attacks via Rotation Transformation

Recent works have demonstrated that deep learning models are vulnerable to backdoor poisoning attacks, where these attacks instill spurious correlations to external trigger patterns or objects (e.g., stickers, sunglasses, etc.). We find that such external trigger signals are unnecessary, as highly effective backdoors can be easily inserted using rotation-based image transformation. Our method constructs the poisoned dataset by rotating a limited amount of objects and labeling them incorrectly; once trained with it, the victim's model will make undesirable predictions during run-time inference. It exhibits a significantly high attack success rate while maintaining clean performance through comprehensive empirical studies on image classification and object detection tasks. Furthermore, we evaluate standard data augmentation techniques and four different backdoor defenses against our attack and find that none of them can serve as a consistent mitigation approach. Our attack can be easily deployed in the real world since it only requires rotating the object, as we show in both image classification and object detection applications. Overall, our work highlights a new, simple, physically realizable, and highly effective vector for backdoor attacks. Our video demo is available at https://youtu.be/6JIF8wnX34M.

==> more_aug.tex <==


\section{More rotation augmentations}
% \label{sec:more_aug}
% For GTSRB, It is also interesting to notice that rotation might change the semantic meanings for some traffic signs (e.g., Drive from the right). Also, some traffic signs are invariant to rotation (e.g., No Entry Sign). Examples are presented in Figure \ref{fig:sign_example}.
% Therefore, it is hard to achieve perfect ASR for multiple source (MC) scenarios.  

% \begin{figure}[t]
% \centering
% \begin{subfigure}{0.5\textwidth}
% \centering
% \includegraphics[width=0.2\linewidth]{Fig/Traffic_sign/80.png} 
% \includegraphics[width=0.2\linewidth]{Fig/Traffic_sign/130.png} 
% \end{subfigure}
% \begin{subfigure}{0.5\textwidth}
% \centering
% \includegraphics[width=0.2\linewidth]{Fig/Traffic_sign/187.png}
% \includegraphics[width=0.2\linewidth]{Fig/Traffic_sign/249.png}
% \includegraphics[width=0.2\linewidth]{Fig/Traffic_sign/883.png}
% \end{subfigure}
% \caption{Examples of rotation invariant signs (up) and Examples which rotation changes semantic meanings (bottom)}
% \label{fig:sign_example}
% \end{figure}




\input{table/temp}

==> table/temp.tex <==
% \usepackage{caption}
% \usepackage{multirow}
% \usepackage{colortbl}
% \usepackage{booktabs}
% \usepackage{hhline}

% \usepackage{caption}
% \usepackage{multirow}
% \usepackage{colortbl}
% \usepackage{booktabs}
% \usepackage{hhline}


\begin{table}
\centering
\setlength{\extrarowheight}{0pt}
\addtolength{\extrarowheight}{\aboverulesep}
\addtolength{\extrarowheight}{\belowrulesep}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\resizebox{16.5cm}{!}{
\begin{tabular}{ccccccccccc} 
\toprule
 & \textbf{} & \textbf{} & \multicolumn{2}{c}{\textbf{15 Degree}} & \multicolumn{2}{c}{\textbf{30 Degree}} & \multicolumn{2}{c}{\textbf{45 Degree}} & \multicolumn{2}{c}{\textbf{90 Degree}} \\ 
\cmidrule[\heavyrulewidth]{3-11}
 & \textbf{} & \begin{tabular}[c]{@{}c@{}}\textbf{Rotation }\\\textbf{Augument}\end{tabular} & \textbf{CDA (\%)} & \textbf{ASR(\%)} & \textbf{CDA (\%)} & \textbf{ASR(\%)} & \textbf{CDA (\%)} & \textbf{ASR(\%)} & \textbf{CDA (\%)} & \textbf{ASR(\%)} \\ 
\bottomrule
\multirow{12}{*}{\textbf{\textbf{GTSRB}}} &  & {[}0, 0] & 97.37 & {\cellcolor[rgb]{0.937,0.937,0.937}}52.59 & 97.45 & {\cellcolor[rgb]{0.937,0.937,0.937}}42.59 & 97.25 & {\cellcolor[rgb]{0.937,0.937,0.937}}79.62 & 97.43 & {\cellcolor[rgb]{0.937,0.937,0.937}}83.33 \\
 & \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{SCA}\\$\rho$= 0.025\%\end{tabular}} & {[}-15, +15] & 97.10 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.00 & 97.69 & {\cellcolor[rgb]{0.937,0.937,0.937}}65.92 & 98.04 & {\cellcolor[rgb]{0.937,0.937,0.937}}85.92 & 97.85 & {\cellcolor[rgb]{0.937,0.937,0.937}}89.62 \\
 &  & {[}-30, +30] & 97.61 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.00 & 96.29 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.00 & 97.60 & {\cellcolor[rgb]{0.937,0.937,0.937}}72.59 & 97.92 & {\cellcolor[rgb]{0.937,0.937,0.937}}97.40 \\
 &  & {[}-45, +45] & 97.02 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.00 & 96.87 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.00 & 97.63 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.00 & 97.35 & {\cellcolor[rgb]{0.937,0.937,0.937}}93.70 \\
 &  & {[}-90, +90] & 96.32 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.00 & 96.27 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.00 & 95.91 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.00 & 96.30 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.00 \\
 &  & {[}-180, +180] & 94.68 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.00 & 93.66 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.00 & 95.27 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.00 & 95.56 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.00 \\ 
\hhline{~~---------}
 & \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{MCA}\\$\rho$= 1.00\%\end{tabular}} & {[}0,0] & 96.72 & {\cellcolor[rgb]{0.937,0.937,0.937}}52.97 & 97.38 & {\cellcolor[rgb]{0.937,0.937,0.937}}77.48 & 97.51 & {\cellcolor[rgb]{0.937,0.937,0.937}}80.15 & 97.31 & {\cellcolor[rgb]{0.937,0.937,0.937}}79.60 \\
 &  & {[}-15, +15] & 97.66 & {\cellcolor[rgb]{0.937,0.937,0.937}}1.09 & 97.79 & {\cellcolor[rgb]{0.937,0.937,0.937}}59.54 & 97.77 & {\cellcolor[rgb]{0.937,0.937,0.937}}82.42 & 97.79 & {\cellcolor[rgb]{0.937,0.937,0.937}}82.23 \\
 &  & {[}-30, +30] & 97.70 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.69 & 97.22 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.98 & 97.75 & {\cellcolor[rgb]{0.937,0.937,0.937}}52.05 & 97.84 & {\cellcolor[rgb]{0.937,0.937,0.937}}82.28 \\
 &  & {[}-45, +45] & 97.50 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.47 & 97.45 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.56 & 97.52 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.81 & 97.18 & {\cellcolor[rgb]{0.937,0.937,0.937}}73.61 \\
 &  & {[}-90, +90] & 96.15 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.54 & 96.18 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.48 & 96.27 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.46 & 96.06 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.48 \\
 &  & {[}-180, +180] & 94.56 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.34 & 94.44 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.29 & 93.17 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.34 & 94.31 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.34 \\ 
\hline\hline
\multirow{12}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Youtube}\\\textbf{Face }\\\textbf{(VGGFace)~}\end{tabular}} &  & {[}0, 0] & 99.90 & {\cellcolor[rgb]{0.937,0.937,0.937}}100.0 & 99.90 & {\cellcolor[rgb]{0.937,0.937,0.937}}100.0 & 99.70 & {\cellcolor[rgb]{0.937,0.937,0.937}}100.0 & 100.0 & {\cellcolor[rgb]{0.937,0.937,0.937}}100.0 \\
 & \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{SCA}\\$\rho$= 0.05\%\end{tabular}} & {[}-15, +15] & 99.80 & {\cellcolor[rgb]{0.937,0.937,0.937}}10.00 & 99.90 & {\cellcolor[rgb]{0.937,0.937,0.937}}100.0 & 99.90 & {\cellcolor[rgb]{0.937,0.937,0.937}}100.0 & 99.90 & {\cellcolor[rgb]{0.937,0.937,0.937}}100.0 \\
 &  & {[}-30, +30] & 99.80 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.00 & 99.90 & {\cellcolor[rgb]{0.937,0.937,0.937}}10.00 & 100.0 & {\cellcolor[rgb]{0.937,0.937,0.937}}100.0 & 100.0 & {\cellcolor[rgb]{0.937,0.937,0.937}}100.0 \\
 &  & {[}-45, +45] & 99.80 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.00 & 99.80 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.00 & 97.30 & {\cellcolor[rgb]{0.937,0.937,0.937}}0.00 & 99.80 & {\cellcolor[rgb]{0.937,0.937,0.937}}100.0 \\
 &  & {[}-90, +90] & 99.80 & {\cellcolor[rgb]{0.937,0.937,0.937}}1.00 & 99.70 & {\cellcolor[rgb]{0.937,0.937,0.937}}4.80 & 99.80 & {\cellcolor[rgb]{0.937,0.937,0.937}}4.20 & 99.80 & {\cellcolor[rgb]{0.937,0.937,0.937}}1.10 \\
 &  & {[}-180, +180] & 99.30 & {\cellcolor[rgb]{0.937,0.937,0.937}}1.00 & 99.80 & {\cellcolor[rgb]{0.937,0.937,0.937}}1.00 & 99.60 & {\cellcolor[rgb]{0.937,0.937,0.937}}1.00 & 99.60 & {\cellcolor[rgb]{0.937,0.937,0.937}}1.00 \\ 
\hhline{~~---------}
 & \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{MCA}\\$\rho$= 1.00\%\end{tabular}} & {[}0, 0] & 99.90 & {\cellcolor[rgb]{0.937,0.937,0.937}}56.40 & 100.0 & {\cellcolor[rgb]{0.937,0.937,0.937}}95.30 & 99.90 & {\cellcolor[rgb]{0.937,0.937,0.937}}99.70 & 100.0 & {\cellcolor[rgb]{0.937,0.937,0.937}}99.80 \\
 &  & {[}-15, +15] & 100.0 & {\cellcolor[rgb]{0.937,0.937,0.937}}33.50 & 99.90 & {\cellcolor[rgb]{0.937,0.937,0.937}}88.20 & 99.90 & {\cellcolor[rgb]{0.937,0.937,0.937}}98.80 & 100.0 & {\cellcolor[rgb]{0.937,0.937,0.937}}100.0 \\
 &  & {[}-30, +30] & 100.0 & {\cellcolor[rgb]{0.937,0.937,0.937}}2.80 & 100.0 & {\cellcolor[rgb]{0.937,0.937,0.937}}53.10 & 100.0 & {\cellcolor[rgb]{0.937,0.937,0.937}}95.90 & 100.0 & {\cellcolor[rgb]{0.937,0.937,0.937}}99.80 \\
 &  & {[}-45, +45] & 100.0 & {\cellcolor[rgb]{0.937,0.937,0.937}}1.30 & 99.90 & {\cellcolor[rgb]{0.937,0.937,0.937}}22.50 & 100.0 & {\cellcolor[rgb]{0.937,0.937,0.937}}58.40 & 99.90 & {\cellcolor[rgb]{0.937,0.937,0.937}}99.50 \\
 &  & {[}-90, +90] & 99.80 & {\cellcolor[rgb]{0.937,0.937,0.937}}1.00 & 99.70 & {\cellcolor[rgb]{0.937,0.937,0.937}}4.80 & 99.80 & {\cellcolor[rgb]{0.937,0.937,0.937}}4.20 & 99.80 & {\cellcolor[rgb]{0.937,0.937,0.937}}1.10 \\
 &  & {[}-180, +180] & 99.30 & {\cellcolor[rgb]{0.937,0.937,0.937}}1.00 & 99.80 & {\cellcolor[rgb]{0.937,0.937,0.937}}1.00 & 99.60 & {\cellcolor[rgb]{0.937,0.937,0.937}}1.00 & 99.60 & {\cellcolor[rgb]{0.937,0.937,0.937}}1.00 \\
\bottomrule
\end{tabular}
}
\caption{Effectiveness of rotation backdoor under data augmentation.(Detailed)}
\label{table:bd_aug_2}
\end{table}



% \usepackage{caption}
% \usepackage{multirow}
% \usepackage{colortbl}
% \usepackage{booktabs}
% \usepackage{hhline}


\begin{table}
\centering
\setlength{\extrarowheight}{0pt}
\addtolength{\extrarowheight}{\aboverulesep}
\addtolength{\extrarowheight}{\belowrulesep}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\resizebox{15cm}{!}{
\begin{tabular}{ccccccccccccccc} 
\toprule
 &  & \textbf{} & \multicolumn{3}{c}{\textbf{15 Degree}} & \multicolumn{3}{c}{\textbf{30 Degree}} & \multicolumn{3}{c}{\textbf{45 Degree}} & \multicolumn{3}{c}{\textbf{90 Degree}} \\ 
\cmidrule[\heavyrulewidth]{3-15}
 &  & \begin{tabular}[c]{@{}c@{}}\textbf{Rotation }\\\textbf{Augument}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{AP}\\\textbf{(\%)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{\textbf{CDR}}\\\textbf{\textbf{(\%)}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{DASR}\\\textbf{(\%)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{\textbf{AP}}\\\textbf{\textbf{(\%)}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{\textbf{\textbf{\textbf{CDR}}}}\\\textbf{\textbf{\textbf{\textbf{(\%)}}}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{\textbf{DASR}}\\\textbf{\textbf{(\%)}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{\textbf{AP}}\\\textbf{\textbf{(\%)}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{\textbf{\textbf{\textbf{CDR}}}}\\\textbf{\textbf{\textbf{\textbf{(\%)}}}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{\textbf{DASR}}\\\textbf{\textbf{(\%)}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{\textbf{AP}}\\\textbf{\textbf{(\%)}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{\textbf{\textbf{\textbf{CDR}}}}\\\textbf{\textbf{\textbf{\textbf{(\%)}}}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{\textbf{DASR}}\\\textbf{\textbf{(\%)}}\end{tabular} \\ 
\bottomrule
\multirow{12}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{\textbf{VOC}} \\\textbf{\textbf{(YOLOR)}}\end{tabular}} & \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{OMA}\\$\rho$= 0.01\%\end{tabular}} & {[}0, 0] & 89.50 & \textcolor[rgb]{0.122,0.122,0.129}{69.00} & {\cellcolor[rgb]{0.937,0.937,0.937}}99.00 & 89.60 & \textcolor[rgb]{0.122,0.122,0.129}{85.20} & {\cellcolor[rgb]{0.937,0.937,0.937}}99.10 & 89.20 & \textcolor[rgb]{0.122,0.122,0.129}{86.00} & {\cellcolor[rgb]{0.937,0.937,0.937}}99.20 & 89.70 & \textcolor[rgb]{0.122,0.122,0.129}{88.10} & {\cellcolor[rgb]{0.937,0.937,0.937}}94.20 \\
 &  & {[}-15, +15] & 88.80 & \textcolor[rgb]{0.122,0.122,0.129}{36.30} & {\cellcolor[rgb]{0.937,0.937,0.937}}96.20 & 88.80 & \textcolor[rgb]{0.122,0.122,0.129}{80.10} & {\cellcolor[rgb]{0.937,0.937,0.937}}98.90 & 88.50 & \textcolor[rgb]{0.122,0.122,0.129}{89.40} & {\cellcolor[rgb]{0.937,0.937,0.937}}98.90 & 88.90 & \textcolor[rgb]{0.122,0.122,0.129}{87.40} & {\cellcolor[rgb]{0.937,0.937,0.937}}\textcolor[rgb]{0.122,0.122,0.129}{90.90} \\
 &  & {[}-30, +30] & 87.70 & \textcolor[rgb]{0.122,0.122,0.129}{32.60} & {\cellcolor[rgb]{0.937,0.937,0.937}}94.60 & 88.00 & \textcolor[rgb]{0.122,0.122,0.129}{62.40} & {\cellcolor[rgb]{0.937,0.937,0.937}}98.10 & 87.90 & \textcolor[rgb]{0.122,0.122,0.129}{76.00} & {\cellcolor[rgb]{0.937,0.937,0.937}}98.40 & 87.90 & \textcolor[rgb]{0.122,0.122,0.129}{88.80} & {\cellcolor[rgb]{0.937,0.937,0.937}}89.40 \\
 &  & {[}-45, +45] & 87.20 & \textcolor[rgb]{0.122,0.122,0.129}{28.30} & {\cellcolor[rgb]{0.937,0.937,0.937}}94.20 & 87.30 & \textcolor[rgb]{0.122,0.122,0.129}{45.40} & {\cellcolor[rgb]{0.937,0.937,0.937}}96.20 & 87.30 & \textcolor[rgb]{0.122,0.122,0.129}{65.50} & {\cellcolor[rgb]{0.937,0.937,0.937}}95.80 & 87.40 & \textcolor[rgb]{0.122,0.122,0.129}{88.40} & {\cellcolor[rgb]{0.937,0.937,0.937}}90.50 \\
 &  & {[}-90, +90] & 84.30 & 50.50 & {\cellcolor[rgb]{0.937,0.937,0.937}}91.60 & 84.50 & 61.00 & {\cellcolor[rgb]{0.937,0.937,0.937}}94.60 & 84.50 & 64.10 & {\cellcolor[rgb]{0.937,0.937,0.937}}93.00 & 85.00 & 48.60 & {\cellcolor[rgb]{0.937,0.937,0.937}}79.10 \\
 &  & {[}-180, +180] & 80.90 & 40.90 & {\cellcolor[rgb]{0.937,0.937,0.937}}91.40 & 81.00 & 68.90 & {\cellcolor[rgb]{0.937,0.937,0.937}}95.10 & 81.00 & 64.20 & {\cellcolor[rgb]{0.937,0.937,0.937}}91.10 & 81.70 & 36.00 & {\cellcolor[rgb]{0.937,0.937,0.937}}75.20 \\ 
\hhline{~--------------}
 & \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{OHA}\\$\rho$= 0.01\%\end{tabular}} & {[}0, 0] & 89.10 & \textcolor[rgb]{0.122,0.122,0.129}{67.60} & {\cellcolor[rgb]{0.937,0.937,0.937}}\textcolor[rgb]{0.122,0.122,0.129}{84.50} & 89.70 & \textcolor[rgb]{0.122,0.122,0.129}{85.20} & {\cellcolor[rgb]{0.937,0.937,0.937}}\textcolor[rgb]{0.122,0.122,0.129}{92.00} & 89.50 & \textcolor[rgb]{0.122,0.122,0.129}{84.60} & {\cellcolor[rgb]{0.937,0.937,0.937}}\textcolor[rgb]{0.122,0.122,0.129}{92.10} & 89.50 & \textcolor[rgb]{0.122,0.122,0.129}{85.90} & {\cellcolor[rgb]{0.937,0.937,0.937}}\textcolor[rgb]{0.122,0.122,0.129}{94.90} \\
 &  & {[}-15, +15] & 88.80 & \textcolor[rgb]{0.122,0.122,0.129}{60.50} & {\cellcolor[rgb]{0.937,0.937,0.937}}\textcolor[rgb]{0.122,0.122,0.129}{66.70} & 89.00 & \textcolor[rgb]{0.122,0.122,0.129}{79.70} & {\cellcolor[rgb]{0.937,0.937,0.937}}\textcolor[rgb]{0.122,0.122,0.129}{82.50} & 88.80 & \textcolor[rgb]{0.122,0.122,0.129}{81.00} & {\cellcolor[rgb]{0.937,0.937,0.937}}\textcolor[rgb]{0.122,0.122,0.129}{93.05} & 88.60 & \textcolor[rgb]{0.122,0.122,0.129}{85.70} & {\cellcolor[rgb]{0.937,0.937,0.937}}\textcolor[rgb]{0.122,0.122,0.129}{96.10} \\
 &  & {[}-30, +30] & 88.10 & \textcolor[rgb]{0.122,0.122,0.129}{57.90} & {\cellcolor[rgb]{0.937,0.937,0.937}}\textcolor[rgb]{0.122,0.122,0.129}{57.40} & 88.00 & \textcolor[rgb]{0.122,0.122,0.129}{76.50} & {\cellcolor[rgb]{0.937,0.937,0.937}}\textcolor[rgb]{0.122,0.122,0.129}{74.00} & 88.00 & \textcolor[rgb]{0.122,0.122,0.129}{78.90} & {\cellcolor[rgb]{0.937,0.937,0.937}}\textcolor[rgb]{0.122,0.122,0.129}{80.10} & 88.30 & \textcolor[rgb]{0.122,0.122,0.129}{85.10} & {\cellcolor[rgb]{0.937,0.937,0.937}}\textcolor[rgb]{0.122,0.122,0.129}{95.10} \\
 &  & {[}-45, +45] & 87.00 & \textcolor[rgb]{0.122,0.122,0.129}{64.70} & {\cellcolor[rgb]{0.937,0.937,0.937}}\textcolor[rgb]{0.122,0.122,0.129}{58.70} & 87.30 & \textcolor[rgb]{0.122,0.122,0.129}{73.40} & {\cellcolor[rgb]{0.937,0.937,0.937}}\textcolor[rgb]{0.122,0.122,0.129}{61.60} & 87.10 & \textcolor[rgb]{0.122,0.122,0.129}{76.00} & {\cellcolor[rgb]{0.937,0.937,0.937}}\textcolor[rgb]{0.122,0.122,0.129}{76.60} & 87.20 & \textcolor[rgb]{0.122,0.122,0.129}{84.10} & {\cellcolor[rgb]{0.937,0.937,0.937}}\textcolor[rgb]{0.122,0.122,0.129}{87.90} \\
 &  & {[}-90, +90] & 84.50 & 65.30 & {\cellcolor[rgb]{0.937,0.937,0.937}}54.90 & 84.70 & 54.60 & {\cellcolor[rgb]{0.937,0.937,0.937}}47.10 & 84.50 & 69.40 & {\cellcolor[rgb]{0.937,0.937,0.937}}55.60 & 84.80 & 35.10 & {\cellcolor[rgb]{0.937,0.937,0.937}}79.10 \\
 &  & {[}-180, +180] & 81.00 & 69.10 & {\cellcolor[rgb]{0.937,0.937,0.937}}46.50 & 81.00 & 74.40 & {\cellcolor[rgb]{0.937,0.937,0.937}}59.80 & 81.00 & 74.40 & {\cellcolor[rgb]{0.937,0.937,0.937}}55.20 & 81.00 & 72.10 & {\cellcolor[rgb]{0.937,0.937,0.937}}44.30 \\
\bottomrule
\end{tabular}
 }
\caption{Effectiveness of rotation backdoor under data augmentation.(Detailed)}
\label{table:bd_aug_od_2}
\end{table}
